Filtered Batch Normalization

It is a common assumption that the activation of different layers in neural networks follow Gaussian distribution. This distribution can be transformed using normalization techniques, such as batch-normalization, increasing convergence speed and improving accuracy. In this paper we would like to demonstrate, that activations do not necessarily follow Gaussian distribution in all layers. Neurons in deeper layers are more selective and specific which can result extremely large, out-of-distribution activations. We will demonstrate that one can create more consistent mean and variance values for batch normalization during training by filtering out these activations which can further improve convergence speed and yield higher validation accuracy.

==> rebuttal.tex <==

Clean version:

The authors are grateful for the constructive comments of the Reviewers to which our detailed responses are given below:

Rev#2:
We have to admit the the improvement of FBN is small, but not insignificant. We afraid we can not provide a fix to further increase FBNs improvement over BN (considering that BN normally results a significant improvement over no normalization at all), we would like to focus on the fact that this improvement is general and was demonstrated with various networks, datasets and tasks and our method has no additional computational cost in inference. We believe based on this even a small but consistent improvement can be helpful in practical applications.
We agree with the reviewer, that filtered group normalization could give better results in Section 4.5. In our manuscript we were focusing on batch normalization and we wanted to demonstrate how filtering can increase accuracy in classification, detection and segmentation. Our approach could possibly be applied on other methods such local or filter response, group normalization, etc. but for that we would like to make more detailed experiments.
According to the suggestion we have executed simulations with filtered group normalization and have final detection AP at 42.27 for detection and 37.65 for segmentation, which are indeed better than the results of batch normalization and we have added these values to Table 1.

Rev#4
We are thankful for the suggestions and have slightly enlarged the text size and the figures of the paper for easier readability, along with a careful perusal to correct every grammatical mistake we could find.
We have to admit, that there is confusion regarding batch-normalization, since in the original paper (Ioffe 2015) mean and variance are calculated for every min-batch separately, in batch re-normalization (Ioffe2017batch) moving averages are stored and the later method is applied in practice.
We have mentioned explicitly in 4.1, that we use and store the moments during training and refer to this algorithm as batch normalization. In our code both batch-normalization and re-normalization (with and without moments) can be found, which also stores the running mean and variance for the filters, but we have used the later in our experiments (as we have stated this in our manuscript).
We have to emphasize the problem we demonstrate is present during training both with and without applying exponential smoothing. If large activations are present, their effect is reduced by the alpha value of the filter (the default value in Pytorch is 0.1), but in case of running average this stationary significant shift will be present for the later batches (even if they do not contain any outliers) due to smoothing which can alter the final value of normalization constants depending on the last training batch.

Rev#5
We completely agree with Rev#5 that our method does not provide such high accuracy as the cited paper. Our aim was not the provide state of the art results, but to demonstrate how filtering out outliers in activations during normalization can improve accuracy. We have presented that our approach could improve accuracy in both batch and group normalization (see the numerical values in the answer to Rev#2). We admit that GN+WS resulted higher accuracy, but our aim is not to compare our method to other approaches, but to demonstrate the effect of our filtering. We also believe that our approach could be used together with weight scaling (also with dropout, data augmentation and other regularization methods), but this was out of scope of the current manuscript.

Rev#6 we are thankful for his/her supporting notes and comments.

Rev #7
Our aim was not to force Gaussian activations, but to keep a consistent output distribution exiting each layer. These distributions are usually considered Gaussian (although as we have demonstrated, it is no entirely true). But keeping the same/similar output distribution is usually implemented by normalizing the mean and the variance. A more detailed answer can be found in (Santurkar 2018) which is cited in our manuscript.
We agree with rev#7 that batch normalization can add significant computation cost in complex networks in training time and we fully agree that our method results increased training time. However, from a practical view-point, the applicability of a network in practice mostly depends on its inference time and would like to emphasize that our method has no additional effect over BN on the inference time of the network.
We completely agree with the third comment of Rev#7 that our work is empirical, but we believe that we have demonstrated on a large enough number of datasets and architectures that the improvement is consistent. Also in the original BN or re-norm papers no theoretical analyses can be found. In our supplementary material we have also demonstrated similar behavior (extremely large activations) in AlexNet, Vgg-16, VGG-19, ResNet50 and ResNext101.


























%
Comments:

Positives:
- The observation of activation outliers and the fix come naturally.
- Ablation experiments are also very diverged and convinced enough to believe FBN is better than BN.


Negatives:
The proposed filtering strategy can be considered as applying the standard z-score based outlier removal for every batch normalization layer. Although the experiments show that the method consistently improves the performance of classification and segmentation, they fail to support their claim as detailed in 5. Overall, I think the novelty is weak and experimental validation is not convincing.

-Significance and novelty
The proposed method removes outlier activations based on z-score in each batch normalization layer. It can be interpreted as a preprocessing step for removing outlier activations for batch normalization. Since it is known that outlier removal as a preprocessing improves performance in general, in my opinion, the observed accuracy improvement in this paper is hard to be regarded as a new finding. Rather, the actual amount of improvement obtainable for specific model architectures and tasks would be more interesting, but they are not provided in this paper.

-It is good that codes are submitted for reproducibility.

-Experimental validation is not sufficient. In the submitted code, filtered batch normalization uses the statics of each mini-batch for normalization during the test time. In contrast, the default settings of the builtin batch normalization in pytorch are as follows:
1) During training, the mean and standard-deviation are calculated each mini-batches.
2) The layer keeps the moving average of mean and variance and updates them during training, which are then used for normalization during evaluation.
Note that the builtin BN and filtered BN are different in two aspects: 1) set of activations used to calculate the statistics during training (whole mini-batch vs. filtered subset) and 2) the statics used during test time (constant statistics tracked during training vs. online estimates during testing). As a result, one cannot conclude from the current experiments that the accuracy gain from BN to filtered BN is obtained from the filtering strategy as claimed in the paper because the effects from two factors cannot be distinguished.

-There are many grammar errors. I suggest careful revision of the manuscript. Also, enlarging text size in the figures would make them more recognizable.




However I found that the quantitative results of the experiments do not meet the previous normalization papers.
For example, in the weight standardization paper [1], MS-COCO Mask-RCNN ResNeXt-101 GN+WS bbox mAP reaches at 43.12 and segm mAP reaches at 38.34.
Meanwhile F-BN's performance is 41.12 for bbox and 37.06 for segm.
Moreover, the performance brought by the filtered BN is significantly less than those of WS (+1.11 vs +6.76 for bbox and +0.59 vs +5.66 for segm), which made me concerned about the effectiveness of F-BN.

Also the proposed approach is naive without analysis on how the filtered BN brings smoother loss landscape than the original batch normalization like lipschitz constant analysis done in [1].
Despite the overall conciseness of the paper, these weaknesses led me to my overall score of this paper.

[1] Qiao, S., Wang, H., Liu, C., Shen, W., & Yuille, A. (2019). Weight standardization. arXiv preprint arXiv:1903.10520.










- The authors provide no justification why forcing the activation distribution to be gaussian can improve results and convergence speed.
- The proposed Filtered Batch Norm requires more computing (doubled). In fact in modern deep learning libraries, the batch norm occupies about 30% - 40% [1]. Thus the proposed technique is not very practical.
- The analysis of the motivation in this work is not theoretically sound. It is mainly based on empirical demonstration that activations are "out-of-distribution" for AlexNet/VGG. This is, however, very limited because we cannot assume all neural networks will behave like AlexNet or VGG.

[1] Restructuring Batch Normalization to Accelerate CNN Training, SysML 2019


In addition to major "merits", here are some additional ones:
+ The experiments of this paper is strong, MNIST/CIFAR/ImageNet/COCO with classification, detection and segmentation. The network architectures include AlexNet/VGG-BN/ResNets. And the results are consistently better.
+ The code submitted is clean and easy to check.

The major weakness of this work is that it appears to be too practical and empirical, and it is not a good match to ICML where more theoretical justifications are more solid and appreciated. For more weaknesses, please check 4. Score Justification.





Qeustions:
- The improvement over BN seems small, can the author(s) elaborate more and speculate which could be the future work to fix.
- In section 4.5, Mask R-CNN seems to work better with Group Norm, should the author(s) provide experiment with GN and FGN into Table 1?








!!!Answers:



- The improvement over BN seems small, can the author(s) elaborate more and speculate which could be the future work to fix.
improvement is small, but not insignificant...referring to reviewer...we think this is general...not major improvement, but can be applied in various fields




- In section 4.5, Mask R-CNN seems to work better with Group Norm, should the author(s) provide experiment with GN and FGN into Table 1?
This si true. Mask-rCNN is a generic framework. This mostly depends on the batch size appleid and the architetcure.
With ResNEXt101 only batches of 2 can be used.that is where groupnorm performs better.


REviewer 4:

The moving avera and the smoothed values are also fonud in our implementation. Out code also conatins BN1dFitleredMoments to calcualte a smoothed value.
This only mitigates the problem. For example default value for moments is 0.1 which meanse ,that if a large activation happens, it shifts the mean value by 0.1 times its original shift, but assuming activaitons with 152 sigma, this is still significant.
Calculate an example for this...

Revier 4 is right that we did not calculate fixed batch values in testing.
But we can do that...


For example, in the weight standardization paper [1], MS-COCO Mask-RCNN ResNeXt-101 GN+WS bbox mAP reaches at 43.12 and segm mAP reaches at 38.34.
Meanwhile F-BN's performance is 41.12 for bbox and 37.06 for segm.

We have only used group normlaizaiotn.
We were not aware of weight standardizaiton. Our method has improved. there is a variance as well...GN our impelmentaiton group norm paper WS paper
Our method coul be applied on weight standradizatio nas well.


Lipschitz contant analysisy

Weights inside big kernels look normal because they produced by backprop from many pseudo-independent(I know,not really independent) activation/gradients as result of central limit theorem.
raining with the L2 penalty can be seen as 'imposing a gaussian prior' on the weights.





- The authors provide no justification why forcing the activation distribution to be gaussian can improve results and convergence speed.
we do not force them to be Gaussian. It is a commony knowledge that they follow Gaussian ...up to some level...we normalize them.
Tlak about inner covaraite shift




- The proposed Filtered Batch Norm requires more computing (doubled). In fact in modern deep learning libraries, the batch norm occupies about 30% - 40% [1]. Thus the proposed technique is not very practical.
We would arguee with that This is about training.
This is true in training our method requires more computation. But has no additional computaiton overhad in inference.


- The analysis of the motivation in this work is not theoretically sound. It is mainly based on empirical demonstration that activations are "out-of-distribution" for AlexNet/VGG. This is, however, very limited because we cannot assume all neural networks will behave like AlexNet or VGG.
we demonstrate dthe same affect on Le-NET5, ResNEt 50, Resnet 101 backbone Mask R-CNN. Although our method is empiricla it builds on batch normalizaiton which was commonyl applied in all networks.
specificity of neurons.



We would like to think the reviewers for they useful comments.






The authors thank the reviewer's assessment and comments, which have been addressed below

The authors are thankful for the reviewer for pointingthisout, raising a valid concern











